Full Reference Video Quality Assessment for Machine Learning-Based Video Codecs

Machine learning-based video codecs have made significant progress in the past few years. A critical area in the development of ML-based video codecs is an accurate evaluation metric that does not require an expensive and slow subjective test. We show that existing evaluation metrics that were designed and trained on DSP-based video codecs are not highly correlated to subjective opinion when used with ML video codecs due to the video artifacts being quite different between ML and video codecs. We provide a new dataset of ML video codec videos that have been accurately labeled for quality. We also propose a new full reference video quality assessment (FRVQA) model that achieves a Pearson Correlation Coefficient (PCC) of 0.99 and a Spearman's Rank Correlation Coefficient (SRCC) of 0.99 at the model level. We make the dataset and FRVQA model open source to help accelerate research in ML video codecs, and so that others can further improve the FRVQA model.

==> boneyard.tex <==
%, particularly due to the unique distortions (shown in Fig.~\ref{fig:solo_demo}) added by ML codecs.
%This shows how ML codecs will ultimately take over as the standard in video compression.

%The gold standard of perceptual quality measurement is the human subjective test, where a number of human viewers watch an uncompressed video and then its compressed version and rate the quality of the compressed video. When this is done across a variety of videos, and with multiple viewers (subjects), these ratings are aggregated to quantify and directly compare the perceptual quality we can expect from different codecs.

 % We are now seeing ML codecs capable of compressing videos ~1.2X \cite{jiahao2022} more than the state-of-the-art H.266, while maintaining the same perceptual quality.
%The rise of machine learning (ML) based video codecs has changed the video compression landscape. In 2021, Li et al.~proposed Deep Contextual Video Compression \cite{liDeepContextualVideo2021} which is $\sim1.3X$ more efficient than H.265, and in 2022, the same group proposed a new model\cite{liHybridSpatialTemporalEntropy2022} which surpassed H.266 by 5\% on average. It took ML codecs less than a year to double the compression rate, while DSP codecs take significantly longer. 

% Video codecs were introduced as early as 1929 \cite{kellnImprovementsRelatingElectric}. More recently, 

%Also, it does not build upon the work in video machine learning, such as SlowFast\cite{feichtenhoferSlowFastNetworksVideo2019} and ViViT\cite{arnabViViTVideoVision2021} which demonstrate much higher performance at almost all video tasks compared to Vanilla 3D convolutional models. 
%Also since the model is trained from scratch, its performance highly depends on the size of the dataset.
%It is also worth noting that training C3DVQA (on 8 NVIDIA V100 GPUs) is at least 80X slower than training a VMAF model on the same data for comparable performance.

%Also like C3DVQA it is trained from scratch so it needs a large dataset to perform well.

%To the author's best knowledge, our work is the first proposal for using pre-trained deep video models, particularly the SlowFast model, for full reference video quality assessment.

% Given the lack of data to train models for assessing the quality of videos encoded by modern ML video codecs, our proposed approach takes advantage of transfer learning, i.e. using large models pre-trained on large datasets, for feature extraction.

% TODO: How to cite the 'A crowdsourcing approach to video qualityassessment' paper
% TODO: Add 5-fold CV std to the table?

%as shown in Fig \ref{fig: temporal aug}. 
% \begin{figure}[H]
% \centering
%   \includegraphics[width= 0.7\columnwidth]{images/temporal aug.png}
%   \caption{Sampling along the temporal axis to augment data}
%   \label{fig: temporal aug}
% \end{figure}

% \textbf{Similarly, during testing, we perform the same spatial and temporal augmentations on each reference-encoded video pair, and then average (arithmetic mean) the results obtained for the augmented versions to get the final predicted quality score.}

%We propose a simple and lightweight, yet effective full reference video quality assessment model, which beats the current state-of-the-art models in video quality assessment achieving a high correlation ($PCC=0.99$, $SRCC=0.99$ at the model level) with subjective quality.

%Given $(x_i,y_i)$ and $(x_j,y_j)$ being a pair from $X$ and $Y$ sets, they considered as concordant when the sort order of $(x_i,x_j)$ agrees with $(y_i,y_j)$ otherwise as discordant. The $\tau$ shows the ratio of the difference between the number of concordant and discordant pairs to the total number of pairs.

% TODO: RMSE (3rd order mapping) + OR should be explained in another sections as well. Would not be better to combine all together in a section like "Evaluation metrics"?

    %\subfloat[\label{fig:vbote:rmse:model}]{\includegraphics[width=0.25\textwidth]{images/n_votes/model_full_rmse.jpg} }
    %\subfloat[\label{fig:vbote:rmse:clip}]{\includegraphics[width=0.25\textwidth]{images/n_votes/clip_full_rmse.jpg} }

%(i.e., tied rank correction considering 95\% CI after \cite{naderiTransformationMeanOpinion2020}) 

%\footnote{As the number of clips is large the tied rank correction using 95\% CI is not required \cite{naderiTransformationMeanOpinion2020}}. 

%\input{tables/results_raw_mapped}
%\input{tables/results_raw_mapped_adj}
%\input{tables/results_5fold}
%\input{tables/results_5fold_no_error}
% \input{tables/ablation_5fold.tex}
% \input{tables/ablation_5fold_checkmarks.tex}

\section{Limitations and Future work / Detailed Analyses}

\label{motion_analysis}
\begin{table}[H]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}CV\\ Split\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean File Size \\ (Mb)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Median File Size\\ (Mb)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MLCVQA \\ (SRCC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}VMAF\\  (SRCC)\end{tabular}} \\ \midrule
0 & 7.727 & 7.265 & 0 & 0 \\
1 & 6.766 & 7.275 & 0 & 0 \\
2 & 4.769 & 4.489 & 0 & 0 \\
3 & 6.335 & 6.191 & 0 & 0 \\
4 & 5.142 & 3.492 & 0 & 0 \\ \bottomrule
\end{tabular}%
}
\caption{Performance (Clip Level) of MLCVQA (our model) and VMAF\cite{li_vmaf_2018}, on different cross-validation splits. We can see how MLCVQA performs better at test splits when there is more motion in the clips compared to splits with lesser motion. The motion is measured by the average of the compressed sizes of the videos in the test split.}
\label{tab:size-vs-srcc}
\end{table}

Since our model utilizes features from deep models pre-trained on video action tasks, we expect and notice a small drop in performance on videos with little or no apparent motion, such as a wide-angle recording of a forest with a camera that slowly moves, or a video with little motion in general, e.g., a video of a beach taken from far (Figure \ref{fig:slow_vid}), where there is little to no relative motion. These videos tend to be almost like still images and are very easy for all codecs to encode (i.e., compress to a very small size without a loss in quality), including for the DSP codecs.
\begin{figure}[H]
\centering
  \includegraphics[width= 3.3in]{images/slow_vid.png}
  \caption{Frames uniformly sampled from one of the test videos (10s duration) in cross-validation split 5, which shows little motion. Frames are ordered clockwise, starting from the top left.}
  \label{fig:slow_vid}
\end{figure}


Dynamic videos (with a lot of motion and action) on the other hand,  are harder for models to compress and obviously comprise the majority of the internet video traffic. Our model produces very accurate quality scores for such videos. We analyze the performance of our approach on the different cross-validation splits. In order to quantify the motion, we tried Temporal Information (TI) \cite{noauthor_itu-t_2020}, which uses the difference in the values of pixels at the same location between consecutive frames, as well as optical flow. Both of these methods are unable to take the motion of the camera into account, resulting in random results, i.e., videos which has low motion end up with high motion measures due to the camera movement. Thus we decided to use the compressed file size as a measure of the amount of general motion in a video. The intuition is a video without a lot of motion is easier to compress thus resulting in a small file size while a video with a lot of motion results in a larger file size. We measure the motion in a test split by averaging the file sizes of videos in a split when compressed using H.264 at the same resolution, frame rate, and quality (as determined by ffmpeg parameters). As shown in Table \ref{tab:size-vs-srcc}, there is a clear correlation between the average amount of motion in a test split vs the performance of our approach. We can also notice how VMAF \cite{li_vmaf_2018} being primarily an image metric performs better on the low-motion splits and worse than our model on the regular splits. 

While videos with minimal motion are a minority subset of the videos on the internet and thus can be treated as out-of-distribution data points, future work to improve the quality assessment on this subset could possibly involve using \cite{zhang_unreasonable_2018} to generate frame-level perceptual scores jointly with our video quality assessment to perform better on all kinds of videos.
- *** future work will mention the problems here and how to improve them


==> other-bib_backup <==
@book{ITU-P910,
    address = {Geneva},
    author = {{ITU-T Recommendation P.910}},
    publisher = {International Telecommunication Union},
    title = {{Subjective video quality assessment methods for multimedia applications}},
    year = {2021}
}
@article{naderi2022-p910,
  title={A crowdsourced implementation of ITU-T P.910},
  author={Naderi, Babak and Cutler, Ross},
  journal={arXiv preprint arXiv:2204.06784},
  year={2022}
}

@inproceedings{naderi2020transformation,
  title={Transformation of mean opinion scores to avoid misleading of ranked based statistical techniques},
  author={Naderi, Babak and M{\"o}ller, Sebastian},
  booktitle={2020 Twelfth International Conference on Quality of Multimedia Experience (QoMEX)},
  pages={1--4},
  year={2020},
  organization={IEEE}
}

@inproceedings{zhang2018perceptual,
  title={The Unreasonable Effectiveness of Deep Features as a Perceptual Metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}


@inproceedings{taimoor2020whyperceputal,
author="Tariq, Taimoor
and Tursun, Okan Tarhan
and Kim, Munchurl
and Didyk, Piotr",
title="Why Are Deep Representations Good Perceptual Quality Features?",
booktitle="ECCV",
year="2020",
publisher="Springer International Publishing",
pages="445--461"
}

@inproceedings{ssim,
  author={Zhou Wang and Bovik, A.C. and Sheikh, H.R. and Simoncelli, E.P.},
  journal={IEEE Transactions on Image Processing}, 
  title={Image quality assessment: from error visibility to structural similarity}, 
  year={2004},
  volume={13},
  number={4},
  pages={600-612},
  doi={10.1109/TIP.2003.819861}}

@INPROCEEDINGS{ms-ssim,
  author={Wang, Z. and Simoncelli, E.P. and Bovik, A.C.},
  booktitle={The Thirty-Seventh Asilomar Conference on Signals, Systems & Computers, 2003}, 
  title={Multiscale structural similarity for image quality assessment}, 
  year={2003},
  volume={2},
  number={},
  pages={1398-1402 Vol.2},
  doi={10.1109/ACSSC.2003.1292216}}

@INPROCEEDINGS{vif,
  author={Sheikh, H.R. and Bovik, A.C.},
  journal={IEEE Transactions on Image Processing}, 
  title={Image information and visual quality}, 
  year={2006},
  volume={15},
  number={2},
  pages={430-444},
  doi={10.1109/TIP.2005.859378}}

@INPROCEEDINGS{dlm,
  author={Li, Songnan and Zhang, Fan and Ma, Lin and Ngan, King Ngi},
  journal={IEEE Transactions on Multimedia}, 
  title={Image Quality Assessment by Separately Evaluating Detail Losses and Additive Impairments}, 
  year={2011},
  volume={13},
  number={5},
  pages={935-949},
  doi={10.1109/TMM.2011.2152382}}

@inproceedings{vmaf,
  title={Toward a practical
perceptual video quality metric},
  author={ Li, Zhi and Aaron,Anne and Katsavounidis, Ioannis and 
Moorthy,Anush and Manohara, Megha},
  booktitle={The Netflix Tech Blog},
  year={vol. 6, 2016},
}
@misc{cisco,
  title = {White Paper: Cisco Complete Forecast Highlights 2022},
  howpublished = {\url{https://www.cisco.com/c/dam/m/en_us/solutions/service-provider/vni-forecast-highlights/pdf/Global_Device_Growth_Traffic_Profiles.pdf}},
  note = {Accessed: 2022-10-23}
}
@misc{torchhub_slowfast,
  title = {TorchHub},
  howpublished = {\url{https://pytorch.org/hub/facebookresearch_pytorchvideo_slowfast/}},
  note = {Accessed: 2022-09-25}
}

@inproceedings{imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}


@InProceedings{kinetics,
author = {Carreira, Joao and Zisserman, Andrew},
title = {Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}

@misc{c3dvqa,
  doi = {10.48550/ARXIV.1910.13646},
  
  url = {https://arxiv.org/abs/1910.13646},
  
  author = {Xu, Munan and Chen, Junming and Wang, Haiqiang and Liu, Shan and Li, Ge and Bai, Zhiqiang},

  title = {C3DVQA: Full-Reference Video Quality Assessment with 3D Convolutional Neural Network},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@ARTICLE{live_dataset,
  author={Seshadrinathan, Kalpana and Soundararajan, Rajiv and Bovik, Alan Conrad and Cormack, Lawrence K.},
  journal={IEEE Transactions on Image Processing}, 
  title={Study of Subjective and Objective Quality Assessment of Video}, 
  year={2010},
  volume={19},
  number={6},
  pages={1427-1441},
  doi={10.1109/TIP.2010.2042111}}


@article{csiq_dataset,
  author    = {Phong V. Vu and
               Damon M. Chandler},
  title     = {ViS3: an algorithm for video quality assessment via analysis of spatial
               and spatiotemporal slices},
  journal   = {J. Electronic Imaging},
  volume    = {23},
  number    = {1},
  pages     = {013016},
  year      = {2014},
  url       = {https://doi.org/10.1117/1.JEI.23.1.013016},
  doi       = {10.1117/1.JEI.23.1.013016},
  timestamp = {Sun, 28 May 2017 13:22:39 +0200},
  biburl    = {https://dblp.org/rec/journals/jei/VuC14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{slowfast,
  author={Feichtenhofer, Christoph and Fan, Haoqi and Malik, Jitendra and He, Kaiming},
  booktitle={2019 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={SlowFast Networks for Video Recognition}, 
  year={2019},
  volume={},
  number={},
  pages={6201-6210},
  doi={10.1109/ICCV.2019.00630}}


@INPROCEEDINGS{vivit,
  author={Arnab, Anurag and Dehghani, Mostafa and Heigold, Georg and Sun, Chen and Lučić, Mario and Schmid, Cordelia},
  booktitle={2021 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={ViViT: A Video Vision Transformer}, 
  year={2021},
  volume={},
  number={},
  pages={6816-6826},
  doi={10.1109/ICCV48922.2021.00676}}


@inproceedings{compressedvqa,
  title={Deep learning based full-reference and no-reference quality assessment models for compressed ugc videos},
  author={Sun, Wei and Wang, Tao and Min, Xiongkuo and Yi, Fuwang and Zhai, Guangtao},
  booktitle={2021 IEEE International Conference on Multimedia \& Expo Workshops (ICMEW)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}  


@inproceedings{compressedvqa_pooling,
author = {Li, Dingquan and Jiang, Tingting and Jiang, Ming},
title = {Quality Assessment of In-the-Wild Videos},
year = {2019},
isbn = {9781450368896},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3343031.3351028},
doi = {10.1145/3343031.3351028},
booktitle = {Proceedings of the 27th ACM International Conference on Multimedia},
pages = {2351–2359},
numpages = {9},
keywords = {in-the-wild videos, content dependency, video quality assessment, temporal-memory effects, human visual system},
location = {Nice, France},
series = {MM '19}
}

@book{howell2009statistical,
  title={Statistical methods for psychology},
  author={Howell, David C},
  year={2009},
  publisher={Cengage Learning}
}
@book{field2013discovering,
  title={Discovering statistics using IBM SPSS statistics},
  author={Field, Andy},
  year={2013},
  publisher={sage}
}

@inproceedings{seufert2019fundamental,
  title={Fundamental advantages of considering quality of experience distributions over mean opinion scores},
  author={Seufert, Michael},
  booktitle={2019 Eleventh international conference on quality of multimedia experience (QoMEX)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@inproceedings{sureal,
  title={Recover subjective quality scores from noisy measurements},
  author={Li, Zhi and Bampis, Christos G},
  booktitle={2017 Data compression conference (DCC)},
  pages={52--61},
  year={2017},
  organization={IEEE}
}

@article{p1401,
  title={P. 1401, Methods, metrics and procedures for statistical evaluation, qualification and comparison of objective quality prediction models},
  author={Rec, ITUT},
  journal={International Telecommunication Union, Geneva, Switzerland},
  year={2012}
}

@INPROCEEDINGS{test-time-aug,
  author={Shanmugam, Divya and Blalock, Davis and Balakrishnan, Guha and Guttag, John},
  booktitle={2021 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={Better Aggregation in Test-Time Augmentation}, 
  year={2021},
  volume={},
  number={},
  pages={1194-1203},
  doi={10.1109/ICCV48922.2021.00125}}


@INPROCEEDINGS{rd-kell,
  author={R. D. Kelln},
  booktitle={British Patent No. 341811}, 
  title={Improvements relating to electric picture transmission system}, 
  year={1929}}
  
@article{jiahao2021,
  title={Deep Contextual Video Compression},
  author={Li, Jiahao and Li, Bin and Lu, Yan},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@inproceedings{jiahao2022,
  title={Hybrid Spatial-Temporal Entropy Modelling for Neural Video Compression},
  author={Li, Jiahao and Li, Bin and Lu, Yan},
  booktitle={Proceedings of the 30th ACM International Conference on Multimedia},
  year={2022}
}

@INPROCEEDINGS{resnet,
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Deep Residual Learning for Image Recognition}, 
  year={2016},
  volume={},
  number={},
  pages={770-778},
  doi={10.1109/CVPR.2016.90}}

==> tables/ablation_5fold.tex <==
\begin{table*}[htbp]
    \caption{Performance of final MLCVQA compared to MLCVQA without different components. Metrics are averaged over 5-fold cross-validation splits. All are compared to the final model. Models that are statistically different at 95\% and 90\% confidence levels are indicated by superscripts \textbf{a} and \textbf{b} respectively.}
    \label{tab:results_5fold_final} 
    \centering
%    \resizebox{\textwidth}{!}{%
        \small
        \begin{tabular}{ l  c c c c    c   c c c c}
        \toprule
         \textbf{Objective}&	 \multicolumn{4}{c}{\textbf{Clip level}} & &  \multicolumn{4}{c}{\textbf{Model level}}\\
        
        \textbf{Model} & {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small \textbf{Tau-b 95\%}} & &
        {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}& {\small \textbf{Tau-b 95\%}} 
        \\ 
        \midrule
MLCVQA                  &      0.94 &      0.94 &                       0.85 &         0.80 &&                       0.99 &       0.99 &                       0.34 &         0.93 \\
MLCVQA-NoAug            &      0.92 &      0.91 &                       1.04 &        0.76 &&                       0.99 &       0.98 &                       0.41 &         0.92 \\
MLCVQA-NoFrameFeat       &      0.92 &      0.91 &                       0.99 &        0.78 &&                       0.99 &       0.98 &  0.46{\textsuperscript{b}} &         0.93 \\
MLCVQA-NoAugNoFrameFeat  &      0.89 &      0.88 &  1.18{\textsuperscript{b}} &        0.74 &&  0.99{\textsuperscript{b}} &       0.98 &  0.52{\textsuperscript{a}} &         0.92 \\
\bottomrule
         % clip level 
%         \multicolumn{10}{l}{\small\textbf{\textsuperscript{a}} Strongly stat sig. (t-test p-value to compare the avg across k-folds is less than 0.05).} 
%         \\
         % Model level
%         \multicolumn{10}{l}{\small\textbf{\textsuperscript{b}} Weakly stat sig.  (t-test p-value to compare the avg across k-folds is between 0.05 and 0.1).}
        \end{tabular}
%    }
\end{table*}

==> tables/backup.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccl|cccl}
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Method\\ (CLIP Level)\end{tabular}}} & \multicolumn{4}{c|}{Raw MOS}                                                                    & \multicolumn{4}{c}{Sureal corrected MOS}                                                        \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                                               & SRCC                     & PCC                      & RMSE            & TAU(TAU\_95)            & SRCC                     & PCC                      & RMSE            & TAU (TAU\_95)           \\ \hline
PSNR                                                                                                & 0.8164 (0.8164)          & 0.7283 (0.7282)          &                 & 0.6306(0.6554)          & 0.8180 (0.8179)          & 0.7303 (0.7304)          &                 & 0.6308(0.6492)          \\
MS-SSIM                                                                                             & 0.9175 (0.9122)          & 0.7725 (0.7731)          &                 & 0.7475(0.7970)          & 0.9171 (0.9118)          & 0.7852 (0.7857)          &                 & 0.7472(0.7850)          \\
VMAF                                                                                                & 0.9452 (0.9452)          & 0.9366 (0.9366)          &                 & 0.8015(0.8288)          & 0.9433 (0.9434)          & 0.9377 (0.9377)          &                 & 0.7963(0.8168)          \\
VMAF (re-trained)                                                                                   & 0.9436 (0.9434)          & 0.9410 (0.9409)          & 0.8893          & 0.7969(0.8229)          & 0.9454 (0.9454)          & 0.9436 (0.9436)          & 0.8585          & 0.7989(0.8213)          \\
C3DVQA                                                                                              &                          &                          &                 &                         & 0.9032 (0.9023)          & 0.9023                   &  1.2374         &  0.7231 (0.7503)        \\
CompressedVQA                                                                                       & 0.9476 (0.9475)          & 0.9439 (0.9439)          & 0.9116          & 0.8109(0.8390)          & 0.9467 (0.9465           & 0.9411 (0.9411)          & 0.9993          & 0.8033(0.8244)          \\
ML-CVQA (w/o Aug)                                                                                   & 0.9248 (0.9250)          & 0.9215 (0.9215)          & 1.1189          & 0.7709(0.7962)          & 0.9333 (0.9335)          & 0.9340 (0.9340)          & 1.0060          & 0.7741(0.7964)          \\
ML-CVQA (Ours with aug)                                                                              & \textbf{0.9547 (0.9548)} & \textbf{0.9603 (0.9603)} & \textbf{0.7656} & \textbf{0.8192(0.8472)} & \textbf{0.9595 (0.9598)} & 0.9671 (0.9670) & \textbf{0.6826} & 0.8272(0.8469)                   \\

ML-CVQA (with NFLX data and Aug)                                                                    &                          &                          &                 &                         & 0.9577 (0.9579)          & \textbf{0.9675 (0.9675)} & 0.7132          & \textbf{0.8239(0.8403)} 



\end{tabular}%
}
\end{table*}


\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccl|cccl}
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Method\\ (Model Level)\end{tabular}}} & \multicolumn{4}{c|}{Raw MOS}                                                                    & \multicolumn{4}{c}{Sureal corrected MOS}                                                        \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                                                & SRCC                     & PCC                      & RMSE            & TAU(TAU\_95)            & SRCC                     & PCC                      & RMSE            & TAU (TAU\_95)           \\ \hline
PSNR                                                                                                 & 0.9133 (0.9128)          & 0.7800 (0.7800)          &                 & 0.8063(0.8127)          & 0.9194 (0.9199)          & 0.7823 (0.7826)          &                 & 0.8063(0.8117)          \\
MS-SSIM                                                                                              & \textbf{0.9896 (0.9903)} & 0.8852 (0.8870)          &                 & \textbf{0.9259(0.9486)} & 0.9878 (0.9894)          & 0.8946 (0.8962)          &                 & 0.9145(0.9575)          \\
VMAF                                                                                                 & 0.9591 (0.9586)          & 0.9652 (0.9652)          &                 & 0.8519(0.8713)          & 0.9628 (0.9626)          & 0.9671 (0.9672)          &                 & 0.8519(0.8589)          \\
VMAF (re-trained)                                                                                    & 0.9841 (0.9840)          & 0.9875 (0.9875)          & 0.4177          & 0.9259(0.9300)          & 0.9896 (0.9895)          & 0.9896 (0.9896)          & 0.3753          & 0.9373(0.9298)          \\
C3DVQA                                                                                               &                          &                          &                 &                         & 0.9701 (0.9733)          & 0.9824                   & 0.7203          &0.8917 (0.9007)          \\
CompressedVQA                                                                                        & 0.9756 (0.9751)          & 0.9760 (0.9760)          & 0.6505          & 0.9031(0.9183)          & 0.9878 (0.9893)          & 0.9783 (0.9784)          & 0.7638          & \textbf{0.9430(0.9282)} \\
ML-CVQA (w/o Augmentation)                                                                           & 0.9750 (0.9753)          & 0.9877 (0.9878)          & 0.6032          & 0.8860(0.9313)          & 0.9805 (0.9817)          & 0.9901 (0.9902)          & 0.4722          & 0.9031(0.9104)          \\
ML-CVQA (Ours with aug)                                                                              & 0.9768 (0.9774)          & \textbf{0.9931 (0.9932)} & \textbf{0.3399} & 0.8917(0.9313)          & 0.9847 (0.9850)          & 0.9926 (0.9926)          & \textbf{0.3116} & 0.9088(0.9134)          \\
ML-CVQA (with NFLX data and Aug)                                                                     &                          &                          &                 &                         & \textbf{0.9896 (0.9896)} & \textbf{0.9929 (0.9929)} & 0.3296          & 0.9316(0.9354)         
       
\end{tabular}%
}
\end{table*}


% I am not sure if this one is needed

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccl|cccl}
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Method\\ (Model Level-Top 10)\end{tabular}}} & \multicolumn{4}{c|}{Raw MOS}                                                                    & \multicolumn{4}{c}{Sureal corrected MOS}                                                        \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                                                       & SRCC                     & PCC                      & RMSE            & TAU(TAU\_95)            & SRCC                     & PCC                      & RMSE            & TAU (TAU\_95)           \\ \hline
PSNR                                                                                                        & 0.9758 (0.9758)          & \textit{0.6095 (0.6107)} &                 & 0.9111(0.8832)          & 0.9636 (0.9726)          & \textit{0.6323 (0.6357)} &                 & 0.8667(0.8706)          \\
MS-SSIM                                                                                                     & 0.9515 (0.9535)          & \textit{0.8293 (0.8370)} &                 & 0.8667(0.8932)          & 0.9394 (0.9564)          & 0.8478 (0.8569)          &                 & 0.8222(0.9597)          \\
VMAF                                                                                                        & \textit{0.6242 (0.6242)} & \textit{0.6792 (0.6811)} &                 & 0.6000(0.5968)          & \textit{0.6121 (0.6079)} & \textit{0.7089 (0.7094)} &                 & 0.5556(0.5804)          \\
VMAF (re-trained)                                                                                           & 0.9636 (0.9636)          & 0.9299 (0.9308)          & 0.4389          & 0.9111(0.9309)          & 0.9515 (0.9483           & \textbf{0.9500 (0.9514)} & 0.3746          & 0.8667(0.9189)          \\
C3DVQA                                                                                                      &                          &                          &                 &                         &                          &                          &                 &                         \\
CompressedVQA                                                                                               & \textbf{0.9879 (0.9879)} & \textbf{0.9531 (0.9540)} & 0.3487          & \textbf{0.9556(0.9309)} & \textbf{0.9879 (0.9848)} & 0.9280 (0.9289)          & 0.2665          & \textbf{0.9556(0.9189)} \\
ML-CVQA (w/o Augmentation)                                                                                  & 0.9394 (0.9483)          & 0.9466 (0.9476)          & 0.7317          & 0.8222(0.9415)          & 0.9273 (0.9179)          & 0.9282 (0.9279)          & 0.4838          & 0.7778(0.8222)          \\
ML-CVQA (Ours)                                                                                              & 0.9394 (0.9544)          & 0.9481 (0.9496)          & \textbf{0.2639} & 0.8222(0.8932)          & 0.9394 (0.9451)          & 0.9421 (0.9420)          & \textbf{0.1893} & 0.8222(0.8315)         
\end{tabular}%
}
\end{table*}




























\begin{table}
  \centering
  \begin{tabular}{lcc}
    \toprule
    Method (MODEL) & OR & OR(Transformed) \\
    \midrule
    PSNR & ? & ? \\
    MS-SSIM  & ? & 0.988 \\
    VMAF & ? &  0.954 \\
    VMAF (retrained) & ? & ? \\
    VQM-VFD & ? & ? \\
    C3DVQA & 0.8076* & 0.2307* \\
    CompressedVQA & * & * \\
    Ours & 0.8076 & 0.3076 \\
    \bottomrule
  \end{tabular}
  \caption{Model level comparison of FRVQA methods on the held out test set (* best results handpicked across all epochs)}
  \label{tab:comparison}
\end{table}


==> tables/results_5fold.tex <==
\begin{table*}[htbp]
    \caption{\textcolor{red}{New- 5 fold results - YH: Team please compare this with the next table and let me know which format is better to keep. I prefer the next one. -- C3DVQA and VMAF row is not final yet}. Performance of ML-CVQA compared to other FRVQA models on predicting subjective DMOS in clip and model levels. }
    
    \label{tab:results_raw_adj} 
    \begin{center}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{ l  c c c c c c   c   c c c c c c}
        \toprule
         \textbf{Objective}&	 \multicolumn{6}{c}{\textbf{Clip level}} & &  \multicolumn{6}{c}{\textbf{Model level}}\\
        
        \textbf{Model} & {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} & &
        {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} 
        \\ 
        \midrule

LPIPS         &  0.84+/-0.02 &  0.88+/-0.01 &  2.28+/-0.08 &  0.75+/-0.02 &  0.88+/-0.01 &  0.71+/-0.02 &&   0.95+/-0.0 &   0.95+/-0.0 &  2.38+/-0.09 &  0.81+/-0.02 &    0.95+/-0.0 &  0.87+/-0.01 \\
MS-SSIM       &  0.69+/-0.02 &  0.75+/-0.05 &  2.48+/-0.05 &  0.82+/-0.02 &  0.75+/-0.05 &   0.6+/-0.04 &&  0.89+/-0.01 &  0.93+/-0.01 &  2.55+/-0.06 &    1.0+/-0.0 &    0.95+/-0.0 &  0.86+/-0.01 \\
C3DVQA        &  0.86+/-0.01 &  0.87+/-0.01 &  1.76+/-0.19 &  0.76+/-0.02 &  0.87+/-0.01 &   0.7+/-0.01 &&  0.96+/-0.01 &  0.95+/-0.01 &   1.5+/-0.23 &   0.9+/-0.03 &   0.95+/-0.01 &  0.86+/-0.01 \\
PSNR          &  0.62+/-0.03 &  0.62+/-0.04 &   2.31+/-0.1 &  0.78+/-0.02 &  0.61+/-0.04 &  0.46+/-0.03 &&  0.79+/-0.02 &  0.86+/-0.01 &  2.21+/-0.09 &  0.86+/-0.02 &   0.87+/-0.01 &  0.75+/-0.02 \\
VMAF          &   0.95+/-0.0 &  0.94+/-0.01 &  0.85+/-0.03 &  0.53+/-0.03 &  0.94+/-0.01 &  0.81+/-0.01 &&   0.98+/-0.0 &  0.97+/-0.01 &  0.49+/-0.04 &  0.63+/-0.05 &   0.97+/-0.01 &   0.9+/-0.01 \\
CompressedVQA &  0.86+/-0.01 &  0.89+/-0.01 &  1.73+/-0.14 &  0.72+/-0.03 &  0.89+/-0.01 &  0.73+/-0.01 &&  0.95+/-0.01 &  0.94+/-0.01 &  1.48+/-0.18 &  0.88+/-0.04 &   0.95+/-0.01 &  0.85+/-0.01 \\
\midrule
ML-CVQA       &  0.92+/-0.02 &  0.91+/-0.02 &  0.99+/-0.14 &  0.46+/-0.05 &  0.91+/-0.02 &  0.78+/-0.04 &&   0.99+/-0.0 &   0.98+/-0.0 &  0.46+/-0.04 &  0.67+/-0.06 &    0.98+/-0.0 &  0.93+/-0.01 \\




            %{\small\textbf{PSNR}} \\
            %{\small\textbf{MS-SSIM}} \\
            %{\small\textbf{LPIPS}} \\
            %{\small\textbf{VMAF}} \\
            %{\small\textbf{VMAF - re-trained (w/o Aug.)}}\\
            %{\small\textbf{VMAF - re-trained (w Aug.)}}\\
            %{\small\textbf{C3DVQA (w/o Aug.)}}\\
            %\textcolor{red}{{\small\textbf{C3DVQA (w Aug.)}}}\\
            %{\small\textbf{CompressedVQA (w/o Aug.)}}\\
            %{\small\textbf{CompressedVQA (w Aug.)}}\\
            %{\small\textbf{ML-CVQA (w/o Aug.) - ours}}\\
            %{\small\textbf{ML-CVQA (w Aug.) - ours}}\\
            
        \bottomrule
        \\
        \\     
        \end{tabular}
    }
    \end{center}
\end{table*}

==> tables/results_5fold_no_error.tex <==
\begin{table*}[htbp]
    \caption{\textcolor{red}{5Fold - mlcvqa without vmaf frame features -- this table is temporarily here for everyone's information}. Performance of ML-CVQA compared to other FRVQA models on predicting subjective DMOS in clip and model levels.}
    
    \label{tab:results_raw_adj} 
    \begin{center}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{ l  c c c c    c   c c c c}
        \toprule
         \textbf{Objective}&	 \multicolumn{4}{c}{\textbf{Clip level}} & &  \multicolumn{4}{c}{\textbf{Model level}}\\
        
        \textbf{Model} & {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small \textbf{Tau 95\%}} & &
        {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}& {\small \textbf{Tau 95\%}} 
        \\ 
        \midrule

LPIPS         &  0.84 (0.03) &  0.88 (0.25) &   2.28 (0.0) &  0.72 (0.21) &&   0.95 (0.0) &   0.95 (0.0) &   2.38 (0.0) &   0.86 (0.0) \\
MS-SSIM       &   0.69 (0.0) &  0.75 (0.03) &   2.48 (0.0) &   0.6 (0.02) &&   0.89 (0.0) &   0.93 (0.0) &   2.54 (0.0) &   0.86 (0.0) \\
C3DVQA        &   0.9 (0.54) &   0.9 (0.78) &  1.28 (0.24) &   0.75 (0.6) &&  0.97 (0.02) &  0.97 (0.21) &  0.97 (0.01) &   0.9 (0.22) \\
PSNR          &   0.62 (0.0) &   0.62 (0.0) &   2.31 (0.0) &   0.46 (0.0) &&   0.79 (0.0) &   0.86 (0.0) &   2.21 (0.0) &   0.75 (0.0) \\
VMAF          &  \textbf{0.95 (0.35)} &  \textbf{0.94 (0.38)} &  \textbf{0.85 (0.38)} &  \textbf{0.81 (0.49)} &&  0.98 (0.08) &   0.97 (0.1) &  0.49 (0.62) &   0.9 (0.18) \\
CompressedVQA &  0.94 (0.52) &  \textbf{0.94 (0.35)} &  1.01 (0.91) &  \textbf{0.81 (0.45)} &&   0.97 (0.0) &  0.96 (0.02) &  0.77 (0.01) &  0.89 (0.02) \\
\midrule
ML-CVQA       &         0.92 &         0.91 &         0.99 &         0.78 &&         \textbf{0.99} &         \textbf{0.98} &         \textbf{0.46} &         \textbf{0.93} \\


            %{\small\textbf{PSNR}} \\
            %{\small\textbf{MS-SSIM}} \\
            %{\small\textbf{LPIPS}} \\
            %{\small\textbf{VMAF}} \\
            %{\small\textbf{VMAF - re-trained (w/o Aug.)}}\\
            %{\small\textbf{VMAF - re-trained (w Aug.)}}\\
            %{\small\textbf{C3DVQA (w/o Aug.)}}\\
            %\textcolor{red}{{\small\textbf{C3DVQA (w Aug.)}}}\\
            %{\small\textbf{CompressedVQA (w/o Aug.)}}\\
            %{\small\textbf{CompressedVQA (w Aug.)}}\\
            %{\small\textbf{ML-CVQA (w/o Aug.) - ours}}\\
            %{\small\textbf{ML-CVQA (w Aug.) - ours}}\\
            
        \bottomrule
        \\
        \\     
        \end{tabular}
    }
    \end{center}
\end{table*}

==> tables/results_raw_mapped.tex <==
\begin{table*}[htbp]
    \caption{Performance of ML-CVQA compared to other FRVQA models on predicting subjective DMOS in clip and model levels. Statistical metrics are calculated after fitting a 3\textsuperscript{rd}order monotonic function on predicted scores per FRVQA model.}
    
    \label{tab:results_raw} 
    \begin{center}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{ l  c c c c c c   c   c c c c c c}
        \toprule
         \textbf{Objective}&	 \multicolumn{6}{c}{\textbf{Clip level}} & &  \multicolumn{6}{c}{\textbf{Model level}}\\
        
        \textbf{Model} & {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} & &
        {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} 
        \\ 
        \midrule
            {\small\textbf{PSNR}} & 0.8074 & 0.8164 & 1.5362 & 0.5617 & 0.8107 & 0.6471 && 0.9154 & 0.9133 & 1.1294 & 0.8148 & 0.9142 & 0.8127\\
            
            {\small\textbf{MS-SSIM}}& 0.9096 & 0.9172 & 1.0820 & 0.4568 & 0.9148 & 0.7742 && 0.9784 & 0.9823 & 0.6145 & 0.5926 & 0.9833 & 0.9255\\
            
            {\small\textbf{VMAF}} & 0.9460 & 0.9452 & 0.8443 & 0.4012 & 0.9423 & 0.8229 && 0.9797 & 0.9585 & 0.5263 & 0.5556 & 0.9623 & 0.8713\\
            {\small\textbf{VMAF - re-trained}} & 0.9413 & 0.9436 & 0.8788 & 0.3457 & 0.9388 & 0.8153 && 0.9881 & \textbf{0.9841\textsuperscript{h}} & 0.4508 & 0.5556 & 0.9838 & 0.9300\\
            {\small\textbf{C3DVQA}} & 0.8849 & 0.8815 & 1.2130 & 0.5802 & 0.8785 & 0.7146 && 0.9889 & 0.9737 & 0.5836 & 0.6667 & 0.9807 & 0.9300\\
            {\small\textbf{CompressedVQA}} & 0.9491 & 0.9476 & 0.8200 & 0.3333 & 0.9425 & 0.8261 && 0.9821 & 0.9756 & 0.4887 & 0.5556 & 0.9773 & 0.9183\\
            {\small\textbf{ML-CVQA (w/o Aug.) - ours}} & 0.9287 & 0.9374 & 0.9727 & 0.4321 & 0.9341 & 0.8072 && 0.9862 & 0.9676 & 0.486 & 0.5926 & 0.9758 & 0.9007\\
            {\small\textbf{ML-CVQA - ours}} & \textbf{0.9625\textsuperscript{a}} & \textbf{0.9569\textsuperscript{b}} & \textbf{0.7222\textsuperscript{c}} & \textbf{0.2654\textsuperscript{d}} & \textbf{0.9557\textsuperscript{e}} & \textbf{0.8492\textsuperscript{f}} && \textbf{0.9932\textsuperscript{g}} & 0.9786 & \textbf{0.3096\textsuperscript{i}} & \textbf{0.3333\textsuperscript{j}} & \textbf{0.9848\textsuperscript{k}} & \textbf{0.9313\textsuperscript{l}}\\
        \bottomrule
        % clip level 
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{a  }} Sig. compared to all but Comp.VQA and VMAF.} & 
        % Model level
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{f}} Sig. compared to all but Comp.VQA and VMAFs.}
        \\
        
        % clip level 
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{b, e}} Only sig. compared to PSNR, MS-SSIM and C3DVQA.} & 
        % Model level
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{g, i, j}} Sig. compared to all.}\\
        
        
        % clip level 
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{c  }}  Sig. compared to all but Comp.VQA.} & 
        % Model level
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{h}} Sig. compared to all but ML-CVQA and MS-SSIM.}
        \\
        
        % clip level 
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{d  }}  Sig. compared to all but Comp.VQA and VMAF re-tra.} & 
        % Model level
        \multicolumn{7}{l}{\small\textbf{\textsuperscript{k, l}} Only sig. compared to VMAF, PSNR, and ML-CVQA(w/o Aug.).}
        \\
        \end{tabular}
    }
    \end{center}
\end{table*}

==> tables/results_raw_mapped_adj.tex <==
% \begin{table*}[htbp]
%     \caption{\textcolor{red}{old 1-fold results}. Performance of ML-CVQA compared to other FRVQA models on predicting subjective DMOS in clip and model levels. Statistical metrics are calculated after fitting a 3\textsuperscript{rd}order monotonic function on predicted scores per FRVQA model. Significant tests with Holm–Bonferroni adjustment.}
    
%     \label{tab:results_raw_adj} 
%     \begin{center}
%     \resizebox{\textwidth}{!}{%
%         \begin{tabular}{ l  c c c c c c   c   c c c c c c}
%         \toprule
%          \textbf{Objective}&	 \multicolumn{6}{c}{\textbf{Clip level}} & &  \multicolumn{6}{c}{\textbf{Model level}}\\
        
%         \textbf{Model} & {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} & &
%         {\small \textbf{PCC}} & {\small \textbf{SRCC}}&	{\small\textbf{RMSE}}&	{\small\textbf{OR}}  & {\small \textbf{SRCC 95\%}}& {\small \textbf{Tau 95\%}} 
%         \\ 
%         \midrule
%             {\small\textbf{PSNR}} & 0.8074 & 0.8164 & 1.5362 & 0.5617 & 0.8107 & 0.6471 && 0.9154 & 0.9133 & 1.1294 & 0.8148 & 0.9142 & 0.8127\\
            
%             {\small\textbf{MS-SSIM}}& 0.9096 & 0.9172 & 1.0820 & 0.4568 & 0.9148 & 0.7742 && 0.9784 & 0.9823 & 0.6145 & 0.5926 & 0.9833 & 0.9255\\
%             {\small\textbf{LPIPS}}& 0.9221 & 0.9293 & 1.0077 & 0.4753 & 0.9273 & 0.7944 & & 0.9642 & 0.9615 & 0.6924 & 0.6667 & 0.9644 & 0.8948 \\ 
%             {\small\textbf{VMAF}} & 0.9460 & 0.9452 & 0.8443 & 0.4012 & 0.9423 & 0.8229 && 0.9797 & 0.9585 & 0.5263 & 0.5556 & 0.9623 & 0.8713\\
%             {\small\textbf{VMAF - re-trained}} & 0.9413 & 0.9436 & 0.8788 & 0.3457 & 0.9388 & 0.8153 && 0.9881 & \textbf{0.9841\textsuperscript{e}} & 0.4508 & 0.5556 & 0.9838 & 0.9300\\
%             {\small\textbf{C3DVQA}} & 0.8849 & 0.8815 & 1.2130 & 0.5802 & 0.8785 & 0.7146 && 0.9889 & 0.9737 & 0.5836 & 0.6667 & 0.9807 & 0.9300\\
%             {\small\textbf{CompressedVQA}} & 0.9491 & 0.9476 & 0.8200 & 0.3333 & 0.9425 & 0.8261 && 0.9821 & 0.9756 & 0.4887 & 0.5556 & 0.9773 & 0.9183\\
%             {\small\textbf{ML-CVQA (w/o Aug.) - ours}} & 0.9287 & 0.9374 & 0.9727 & 0.4321 & 0.9341 & 0.8072 && 0.9862 & 0.9676 & 0.4860 & 0.5926 & 0.9758 & 0.9007\\
%             {\small\textbf{ML-CVQA - ours}} & \textbf{0.9625\textsuperscript{a}} & \textbf{0.9569\textsuperscript{b}} & \textbf{0.7222\textsuperscript{c}} & \textbf{0.2654\textsuperscript{a}} & \textbf{0.9557\textsuperscript{b}} & \textbf{0.8492\textsuperscript{b}} && \textbf{0.9932\textsuperscript{d}} & 0.9786 & \textbf{0.3096\textsuperscript{d}} & \textbf{0.3333\textsuperscript{d}} & \textbf{0.9848\textsuperscript{f}} & \textbf{0.9313\textsuperscript{e}}\\
%         \bottomrule
%         % clip level 
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{a}} Sig. compared to all but Comp.VQA and VMAFs.} & 
%         % Model level
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{d}} Sig. compared to all.}
%         \\
        
%         % clip level 
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{b}} Only sig. compared to PSNR, MS-SSIM and C3DVQA.} & 
%         % Model level
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{e}} Only sig. compared to PSNR, VMAF and ML-CVQA(w/o Aug.).}\\
        
        
%         % clip level 
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{c     }}  Sig. compared to all but Comp.VQA and VMAF.} & 
%         % Model level
%         \multicolumn{7}{l}{\small\textbf{\textsuperscript{f}} Only sig. compared to PSNR and VMAF.}
%         \\
        
%         \end{tabular}
%     }
%     \end{center}
% \end{table*}
